Bi-Manual Manipulation and Attachment via Sim-to-Real Reinforcement Learning

Most successes in robotic manipulation have been restricted to single-arm robots, which limits the range of solvable tasks to pick-and-place, insertion, and objects rearrangement. In contrast, dual and multi arm robot platforms unlock a rich diversity of problems that can be tackled, such as laundry folding and executing cooking skills. However, developing controllers for multi-arm robots is complexified by a number of unique challenges, such as the need for coordinated bimanual behaviors, and collision avoidance amongst robots. Given these challenges, in this work we study how to solve bi-manual tasks using reinforcement learning (RL) trained in simulation, such that the resulting policies can be executed on real robotic platforms. Our RL approach results in significant simplifications due to using real-time (4Hz) joint-space control and directly passing unfiltered observations to neural networks policies. We also extensively discuss modifications to our simulated environment which lead to effective training of RL policies. In addition to designing control algorithms, a key challenge is how to design fair evaluation tasks for bi-manual robots that stress bimanual coordination, while removing orthogonal complicating factors such as high-level perception. In this work, we design a Connect Task, where the aim is for two robot arms to pick up and attach two blocks with magnetic connection points. We validate our approach with two xArm6 robots and 3D printed blocks with magnetic attachments, and find that our system has 100% success rate at picking up blocks, and 65% success rate at the Connect Task.

==> 1200_future_work.tex <==
\section{Limitations, Discussion \& Future Directions}
We introduced an enhancement for simulations that enables MLP agent to learn joint space control for bi-arm collaborative object manipulation tasks which can handle perception noises, actuation noises, inverse kinematics and collision detection via large-scale RL.  While our work showed that a solution to our objective exists, it is by no means efficient - requiring 2 billions steps of training.  To address more complex bi-manual tasks than the connect task, it is likely that the training time can be shortened by structured RL like graph neural net, or transformer architecture.  Imitation learning by using already trained policy is also a possible solution to improve training time.

==> 1420_train_plots.tex <==
\begin{figure}[H]
    \centering
    \includegraphics[scale=.17]{images/pick_success.png}
    \includegraphics[scale=.17]{images/pick_return.png}
    \caption{
        \small{
            Pickup Task Training Progress.
        }
    }
    \label{fig:pick_progress}
\end{figure}
\begin{figure}[H]
    \centering
    \includegraphics[scale=.17]{images/connect_success.png}
    \includegraphics[scale=.17]{images/connect_return.png}
    \caption{
        \small{
            Connect Task Training Progress.
        }
    }
    \label{fig:connect_progress}
\end{figure}

==> bak_0100_abstract.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{abstract}
\kg{the current state of abstract has too much details, and way too long. Need to come back to this and fix.}

Learning \kg{what do you mean by soft?} \sk{In robotics industry, typically realtime means "hard" realtime which is extremely low latency like less than 100ns and also deterministic for 1000-5000Hz control.  Soft real-time is like gaming level, 1-60Hz.  Some robotics orientated people cause an alleegy when talking about soft real-time without mentioning it.} \kg{In my experience, soft can refer to many things like deformable objects, soft grippers, or even compliant control. So better to use a more accurate terminology.} \sk{I see.  Then how about using semi real-time?} soft real-time joint control policy for bi-manual collaborative object manipulation tasks with reinforcement learning (RL) is both a valuable functionality for autonomous robotics, as well as a valuable diagnostic task for open-ended training of embodied intelligent agents.  Though RL with neural networks is a powerful approach owing to its general versatility, RL training happens in simulator because it takes billions of environment steps which amount is unrealistically large in the real world.  In particular, 2 billion environment steps are equivalent to 5787 days of robot operation time.  Also, given that training data of 2 billion environment step can be produced in 24 hours using 3000CPUs, we need to run at least 5 thousand real robots in parallel if we want to achieve the same training performance by using real robots.  However, joint control policies trained in simulator rarely perform well when executed on real robotics hardware, even if specifications are correct.
Specifically, training RL model for soft real-time joint control in simulation is hard to be transferred to the real world because perception noises, actuation noises and actuator constraints of the real world environments are not correctly reproduced in simulators.  Also bi-manual collaborative manipulation tasks are naturally more challenging than the single arm tasks due to additional complexities from doubled DoF, severe timing requirements for two arm synchronization and accuracy requirements for object manipulation.
% \kg{here describing challenges of bimanual} done.
In addition to the noises, manipulating objects using multiple robotics arms easily causes perception occlusions, and also the arms easily collide each other when collaborating each other.  The gap between simulated environment and real world world environment causes significant accuracy reduction for soft real-time behaviors from the RL policy trained in simulation.  The aim of this work is to sutdy how RL controllers can be trained for bimanual robotic tasks, and critically, transferred to the real world.
% \kg{The aim of this work is... Studying how RL controllers can be trained for bimanual robotic tasks, and critically, transferred to the real world}
To solve our objective, we introduced a naturalistic physics-based environment with connectable magnet blocks which enables our agent to reproduce the RL control in the real world.
% \kg{which is reproducible in the real world}. \kg{the tasks and why they are hard}
In this paper, we define two tasks using toy blocks 1. two block connecting task as our major goal and 2. one block picking-up task as a preliminary step toward the connect task.  Despite its simplicity of the connect task, training neural network models for soft real-time joint control is hard because the task requires: 1. accuracy for connecting blocks to be right a desired structure, 2. timing synchronization for collaborative bi-arm manipulation, 3. collision free joint behavior.  The composite complexity of these requirements and environmental noises in the real world prevents the joint space control agent from solving the task in real world when being trained on a simulated environment.
% makes the training in simulation 
% on top of the difficulties mentioned above.
% as the neural network agent needs to 
% 1. single block pick-up task with a robotics arm 2. two block connect task with two robotics arms.  
% Despite the simplicity of these tasks, training neural network model for soft-realtime joint control for multiple robotics arms becomes exponentially costly as it needs to produce collision free poses with noisy perceptions and noisy actuation.  Specifically, two block connect task requires 
% accurate behavior and timing synchronization between two robotics arms.
% which combination makes the training significantly harder than a single manipulation tasks.
% \kg{the solution and findings}
Through our study toward the connect task in the real world, we found that the combination of our simulation enhancement and large scale RL can train neural network model for joint space control which can successfully solve the connect task with environmental noises in the real world.  In particular, we added realistic physical noises on top of the physics mujoco simulator which are specifically important to train RL policies to generate feasible soft-realtime trajectories. Furthermore, since the policy generates joint trajectories, the policy output is directly fed into robot controllers without being translated from Cartesian poses via neither trajectory generation middleware nor IK function.  This approach is aiming at reducing possible gaps between simulator and on-robot software stack, this helps agents train in simulation more effectively.  This also helps the simulator reproduce realistic constraints, in particular, simulators can constraint joint velocity and acceleration directly.  While joint space control provides larger control space than Cartesian space control which enables bi-manual control a lot, joint space control RL requires larger computational resources due to the different of the action space size.  We find that large-scale reinforcement learning with MLP can train neural network for bi-arm manipulation joint control.  Through extensive experiments, we highlight the importance of perception noises, actuation noises and acceleration constraints and discuss contributions of them for real world demonstration.  We hope this work further encourages study of large-scale RL for sim-to-real.
% \kg{We hope...}
\end{abstract}
% Also, we added realistic physical noises on top of the physics mujoco simulator which are specifically important to train RL policies to generate feasible soft-realtime trajectories.  In this paper, we define two task using toy blocks 1. single block pick-up task with a robotics arm 2. two block connect task with two robotics arms.  Despite the simplicity of these tasks, training neural network model for soft-realtime joint control for multiple robotics arms becomes exponentially costly as it needs to produce collision free poses with noisy perceptions and noisy actuation.  Furthermore, since the policy generates joint trajectories, the policy output is directly fed into robot controllers without being translated from Cartesian poses via neither trajectory generation middleware nor IK function.  This approach is aiming at reducing possible gaps between simulator and on-robot software stack, this helps agents train in simulation more effectively.  This also helps the simulator reproduce realistic constraints, in particular, simulators can constraint joint velocity and acceleration directly.  While joint space control provides larger control space than Cartesian space control which enables bi-manual control a lot, joint space control RL requires larger computational resources due to the different of the action space size.  We find that large-scale reinforcement learning with MLP can train neural network for bi-arm manipulation joint control.  Through extensive experiments, we highlight the importance of perception noises, actuation noises and acceleration constraints and discuss contributions of them for real world demonstration.
